A Multi-Level Task Framework for Event Sequence Analysis

Despite the development of numerous visual analytics tools for event sequence data across various domains, including but not limited to healthcare, digital marketing, and user behavior analysis, comparing these domain-specific investigations and transferring the results to new datasets and problem areas remain challenging. Task abstractions can help us go beyond domain-specific details, but existing visualization task abstractions are insufficient for event sequence visual analytics because they primarily focus on multivariate datasets and often overlook automated analytical techniques. To address this gap, we propose a domain-agnostic multi-level task framework for event sequence analytics, derived from an analysis of 58 papers that present event sequence visualization systems. Our framework consists of four levels: objective, intent, strategy, and technique. Overall objectives identify the main goals of analysis. Intents comprises five high-level approaches adopted at each analysis step: augment data, simplify data, configure data, configure visualization, and manage provenance. Each intent is accomplished through a number of strategies, for instance, data simplification can be achieved through aggregation, summarization, or segmentation. Finally, each strategy can be implemented by a set of techniques depending on the input and output components. We further show that each technique can be expressed through a quartet of action-input-output-criteria. We demonstrate the framework's descriptive power through case studies and discuss its similarities and differences with previous event sequence task taxonomies.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Sections/figure.tex <==
\usepackage{multirow}
\usepackage{rotating}
\section{Fig1: Intent, Strategy, Technique}


\begin{table}[htbp]
    \centering
    \begin{tabular}{l|c|c|c|c|c}
    \hline
    \multicolumn{11}{c|}{Augment Data}
    & \multicolumn{9}{c|}{*}{Simplify Data}
    & \multicolumn{6}{c|}{Configure Data}
    & \multicolumn{8}{c|}{Configure Visualization} 
    & \multicolumn{3}{c|}{Create Provenance} \\
    
    \end{tabular}
    \label{tab:multirow-multicolumn}

\end{table}

==> Sections/mappingtoprevious.tex <==
\subsection{Mapping to Previous Work}
\hannah{add an introduction}

\zinat{May or may not add to rebuttal}
Here, we provide a detailed discussion about the difference between our framework and previous ones. 

\subsubsection{Comparison to Task Typology for Time-Stamped Event Sequences}

A fundamental difference between our framework and Peiris et al. \cite{peiris2022data} lies in the structure. While our framework organizes tasks into a four-level hierarchy, and a quartet for the lowest level, Peiris et al. employ a flat structure, where each task is characterized in three dimensions: action, target, and criteria. 

A comparative analysis of our task framework and the typology proposed by Peiris et al. \cite{peiris2022data} reveals significant overlap in the covered quartets and triplet categories. Many of the actions identified in Peiris et al.'s typology,
such as `Summarize', `Group', `Segment', `Annotate', and `Show Details', have clear equivalents in our framework, indicating a shared understanding of the fundamental tasks involved in event sequence analysis. \hannah{I'm a bit confused here in one sentence, you talk about overlapping tasks but don't mention which ones and in the next sentence, you start talking about actions. I feel like there needs to be a transition sentence in between to make the writing clearer..}

However, a closer examination of the two frameworks highlights a key difference in the categorization of tasks. Peiris et al.'s typology intermixes tasks at different levels of abstraction, with some actions corresponding to our high-level objectives (e.g., `Compare', `Identify Common', `Analyze State Transition', and `Detect Outliers/Anomalies'), some mapping to mid-level strategies(`Summarize', `Group', `Segment') and others aligning with our lower-level techniques (`Predict', `Sort/Rank', `Annotate'). In contrast, our framework provides a clearer separation of tasks into a four-level hierarchy. This hierarchical abstraction allows for a more systematic organization of tasks. \hannah{I would rearrange this paragraph. After the sentence mentioning that Peiris et al. intermix tasks, immediately contrast it with your framework. Then, give specific instances where you make distinctions in the hierarchy and explain why your approach is better. Basically decenter the Peiris typology from the narrative here and focus on highlighting where your own work stands out.}
% based on their level of abstraction and purpose.

Furthermore, our framework includes several tasks related to data transformation and pattern mining, such as `Create Event Hierarchy', `Extract Common Patterns', and `Extract Latent Patterns', which are not explicitly present in Peiris et. al.'s typology. 
% Conversely, Peiris et. al. mentions tasks like `Recommend'  which do not have a direct equivalent in our paper. We identify it as a potential low-level technique under strategy `simulate', but since our technique list is not exhaustive, it is not included in the paper.


For low-level techniques, we use an action-input-output-criteria quartet compared to Peiris et. al.'s ction-target-criteria triplet, providing a more detailed breakdown of each technique components.

Another notable difference between the two frameworks lies in their treatment of targets and criteria. In Peiris et al., targets and criteria are expressed as a fixed set of data characteristics, with four types of targets and five types of criteria. However, we believe that input (analogous to targets) and criteria are too expansive to be limited to a predefined set of elements. Peiris et al. also states that `criteria describe the means to perform an action', but map it solely to data components. Whereas, we view criteria as not necessarily being data components but potentially including procedures for executing techniques.

\hannah{One thing that could help would be highlighting each difference you discuss in the paragraphs. One way would be to introduce summary paragraph headings. Alternatively, you could just bold each key difference.}

\zinat{Mention the TSES has a broad category named feature for criteria, we however think it's not the correct granularity/ criteria is too expansive to be limited into fixed set of elements. Also TSES says: Like targets, criteria are typically a data characteristics. In contrast to targets, criteria describe the means to perform an action. Criteria for us is not necessarily data component, it can be a procedure for executing a technique}


\subsubsection{Comparison with Du et. al}

Many of Du et al.'s strategies \cite{du2016volumeandvariety} align with techniques under the Augment Data and Simplify Data intents in our framework. Seven of their proposed extraction and iterative strategies, like (`Goal-Driven Record Extracting' $\rightarrow$ `Execute Dynamic Queries') with variations in input-output-criteria combination \hannah{this sentence is confusing}.  Their temporal folding and pattern simplification strategies,
like `Grouping Event Categories'
`Coalescing Repeating Point Events into One', also have clear counterparts in our framework. This overlap suggests that both works recognize the fundamental importance of data processing tasks like extracting, aligning, folding and aggregating for event sequence data.

However, the two frameworks also differ in their scope and emphasis. Du et al. \cite{du2016volumeandvariety} focus primarily on data-centric strategies, while our framework takes an end-to-end view that encompasses visual encoding, interaction and provenance techniques.  Also, the proposed strategies are equivalent to our technique and can be mapped to action-input-output-criteria quartet, higher level intents or strategies are not present in Du et al.'s strategies \hannah{the last part of this sentence seems important and should be discussed more}.

\subsubsection{Comparison with Plaisant et. al}
\label{subsec:comp}

Plaisant et. al. \cite{plaisant2016diversity} identifies eight high-level user tasks for event sequence analysis and groups them into three categories. Four of their mentioned tasks map to    `objective' level in our framework (e.g., `Find and describe deviations from required or expected patterns' $\rightarrow$ Anomaly detection), which is consistent with their tasks being termed as high level. Other high-level goals  are either mapped to intents and strategies (e.g., identify a set of records of interest $\rightarrow$ Include-Exclude) or can be implemented through a mix of strategies (e.g., Compile descriptive information about the dataset or a subgroup of records and events $\rightarrow$ \{Summarize, Organize\}). Compared to our framework, the task list primarily focuses on data analysis goals and doesn't explicitly cover  provenance or visualization tasks. Plaisant et. al.'s task list \cite{plaisant2016diversity} provides a general description of analysis goals without delving into lower-level details, making it more challenging to directly map to specific techniques.


==> Sections/table.tex <==
\begin{table*}[!t]\fontfamily{ptm}\selectfont\small
\caption{Comparative analysis of task mappings for three case study excerpts (SeqCausal \cite{jin2021seqcausal}, RASIPAM \cite{wu2022rasipam} and FlexEvent \cite{linden2023flex}) using our multi-level task framework and existing task taxonomies (Plaisant et al. \cite{plaisant2016diversity}, Du et al. \cite{du2016volumeandvariety}, Peiris et al. \cite{peiris2022data}). The color scheme indicates the level of alignment: \textcolor{Red3}{no match} and \textcolor{magenta}{partial match}. Our framework demonstrates more comprehensive mapping compared to existing taxonomies
}
\label{tbl:case1}
% \centering
{\small
\begin{tabular}{p{0.25\linewidth}
p{0.14\linewidth}
p{0.12\linewidth}
p{0.16\linewidth}
p{0.25\linewidth}}
\hline
Example Excerpt  & Plaisant et al. \cite{plaisant2016diversity} &  Du et al. \cite{du2016volumeandvariety} & Peiris et al. \cite{peiris2022data} & Ours \\
\hline
 \textbf{T1} \cite{jin2021seqcausal} \textit{The doctors queried a group of $127$ middle-aged patients aging from $50$ to $60$ who were diagnosed
with pneumonia}. & Identify a set of records of interest & Goal-Driven Record Extracting & 
action: Filter\newline
target: Event Sequences\newline
criteria: Metadata Attributes 
% \begin{tabular}[c]{@{}l@{}} action: Filter\\target: Event Sequences\\criteria: MetaData Attributes \end{tabular}  
& 
Intent: Configure Data\newline
Strategy: Include-Exclude\newline
Technique: Execute Dynamic Queries\newline
action: Query \newline
input: Event Sequences \newline
output: Filtered Event Sequences \newline criteria: Age
% \begin{tabular}[c]{@{}l@{}}Intent: Configure Data\\Strategy: Include-Exclude\\Technique: Execute Dynamic Queries\end{tabular}
% Intent: Configure Data; Strategy: Include-Exclude; Technique:Execute Dynamic Queries 
\\
\hline
 \textbf{T2} \cite{jin2021seqcausal} \textit{After several iterations of confirming causalities and model updates}, $\dots$ & Review data quality and inform choices to be made in order to model the data  & \textcolor{Red3}{n/a} &
 % \begin{tabular}[c]{@{}l@{}} action: Derive Metrics\\target: \textcolor{Red3}{n/a}\\criteria: \textcolor{Red3}{n/a} \end{tabular} 
 action: Derive Metrics\newline
 target: \textcolor{Red3}{n/a}\newline
 criteria: \textcolor{Red3}{n/a}
 &
 Intent: Configure Data\newline
 Strategy: Refine\newline
 Technique: Adjust Parameters \newline
 action: Adjust \newline input:  Current causal model \newline
 output: Updated causal model \newline
 criteria: Domain knowledge
 % \begin{tabular}[c]{@{}l@{}}Intent: Configure Data\\Strategy: Refine\\Technique: Adjust Parameters\end{tabular}
 % Intent: Configure Data; Strategy: Refine; Technique: Adjust Parameters 
 \\
\hline
% The doctors confirmed the causality circle $\dots$  & Review data quality and inform choices to be made in order to model the data & \textcolor{red}{n/a} & \textcolor{magenta}{Action: Derive Metrics}  & Intent:  Configure Data, Strategy: Refine, Technique: Adjust Parameters \\
% \hline
  \textbf{T3} \cite{jin2021seqcausal} $\dots$ \textit{the doctors saved the final causality to the analysis history view}    & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & 
  % \begin{tabular}[c]{@{}l@{}} action: \textcolor{magenta}{Annotate}\\target: \textcolor{Red3}{n/a}\\criteria: \textcolor{Red3}{n/a} \end{tabular} 
  action: \textcolor{magenta}{Annotate} \newline target: \textcolor{Red3}{n/a} \newline criteria: \textcolor{Red3}{n/a}
  & 
  Intent: Create Provenance \newline
  Strategy: Document \newline
  Technique: Save/Record Analysis \newline
  action: Save/Record \newline input:  Analysis State \newline
 output: Saved/Recorded Analysis \newline
 criteria: User-specified snapshot
  % \begin{tabular}[c]{@{}l@{}}Intent: Create Provenance\\Strategy: Document\\Technique: Save/Record Analysis\end{tabular}
  % Intent: Create Provenance, Strategy: Document, Technique: Save/Record Analysis 
  \\
\hline
 \textbf{T4} \cite{wu2022rasipam} \textit{E2 re-ranked the tactics in Tactic View based on the tactical importance } $\dots$  & \textcolor{magenta}{Identify a set of records of interest}  & \textcolor{Red3}{n/a} & 
 action: {Sort/Rank} \newline target: \textcolor{magenta}{Event Sequences} \newline criteria: Metrics/Features & 
 Intent: Configure Visualization \newline Strategy: Rearrange\newline Technique: Reorder/Sort Components \newline
 action: Reorder/Sort \newline input:  Tactics \newline
 output: Reordered Tactics \newline
 criteria: Tactical importance metric
 % \begin{tabular}[c]{@{}l@{}}Intent: Configure Visualization\\Strategy: Rearrange\\Technique: Reorder/Sort Components\end{tabular}
 % Intent: Configure Visualization, Strategy: Rearrange, Technique: Reorder/Sort Components 
 \\
\hline
 \textbf{T5} \cite{wu2022rasipam} \textit{Experts applied this merging adjustment  and obtained a
more accurate estimate of the win rate for this serving tactic.}   & Review data quality and inform choices to be made in order to model the data \newline Identify a set of records of interest & \textcolor{Red3}{n/a} & 
 action: Add/Modify \textcolor{magenta} \newline target: \textcolor{magenta}{Event Sequences} \newline criteria: Metrics/Features & 
 Intent: Configure Data\newline
 Strategy: Refine\newline
 Technique: Modify Summary \newline
 action: Modify \newline input:  Tactics \newline
 output: Modified Tactics \newline
 criteria: Domain knowledge
 % \begin{tabular}[c]{@{}l@{}}Intent: Configure Data\\Strategy: Refine\\Technique: Modify Summary\end{tabular}
 % Intent: Configure Data, Strategy: Refine, Technique: Modify Summary 
 \\
\hline
\multirow{ 2}{*}{\shortstack[l]{\textbf{T6} \cite{linden2023flex} $\dots$ selected 22 attributes of interest\\ for dimensionality reduction with clustering}}
% {\textbf{T6} \cite{linden2023flex} $\dots$ selected 22 attributes of interest for dimensionality reduction with clustering} 
& Review data quality and inform choices to be made in order to model the data  
& \textcolor{Red3}{n/a} & action: Derive Metrics \newline target: Metadata Attributes \newline criteria: \textcolor{Red3}{n/a}    & 
Intent: Augment Data\newline 
Strategy: Derive\newline 
Technique: Obtain Embeddings/ Projections
\newline
 action: Obtain \newline input:  Attributes \newline
 output: Projections \newline
 criteria: t-SNE \\
% \begin{tabular}[c]{@{}l@{}} Intent: Augment Data\\ Strategy: Derive\\ Technique: Obtain Embeddings/ Projections \end{tabular} 
\cline{2-5}
& Identify a set of records of interest  & \textcolor{Red3}{n/a} & 
 action: Group \newline target:\textcolor{Red3}{n/a} \newline criteria: \textcolor{Red3}{n/a} & Intent: Augment Data\newline Strategy: Organize\newline Technique: \textcolor{magenta}{Group Sequences} \newline
 action: Group \newline input:  \textcolor{Red3}{n/a} \newline
 output: \textcolor{Red3}{n/a} \newline
 criteria: clustering  \\
\hline
%  \textbf{T6} \cite{linden2023flex} \textit{using grouping on (non-)sepsis patients} $\dots$  & \textcolor{magenta}{Identify a set of records of interest}  & \textcolor{red}{n/a}  & action: Group, target: Event Sequences (patients),
% criteria: Metadata Attribute
%    & 
%    \begin{tabular}[c]{@{}l@{}}Intent: Augment Data\\Strategy: Organize\\Technique: Group Sequences\end{tabular}
%    % Intent: Augment Data, Strategy: Organize, Technique: Group
   % \\
   % \hline
    \textbf{T7} \cite{linden2023flex} \textit{changing the color attribute to sepsis}, $\dots$  & \textcolor{Red3}{n/a}  & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & 
    % Intent: Configure Visualization, Strategy: Visualize, Technique: Produce Visualization 
    \begin{tabular}[c]{@{}l@{}}Intent: Configure Visualization\\Strategy: Visualize\\Technique: Produce Visualization\end{tabular}
    \\
\hline
\end{tabular}}
\end{table*}


==> Sections/table2.tex <==
\begin{table*}[!t]\fontfamily{ptm}\selectfont\small
\caption{Comparative analysis of task mappings for three case study excerpts (SeqCausal \cite{jin2021seqcausal}, RASIPAM \cite{wu2022rasipam} and FlexEvent \cite{linden2023flex}) using our multi-level task framework and existing task taxonomies (Plaisant et al. \cite{plaisant2016diversity}, Du et al. \cite{du2016volumeandvariety}, Peiris et al. \cite{peiris2022data}). The color scheme indicates the level of alignment: \textcolor{Red3}{no match} and \textcolor{magenta}{partial match}. Our framework demonstrates more comprehensive mapping compared to existing taxonomies}
\label{tbl:case1}
% \centering
{\small
\begin{tabular}{p{0.03\linewidth}
p{0.1\linewidth}
p{0.1\linewidth}
p{0.13\linewidth}
p{0.11\linewidth}
p{0.115\linewidth}
p{0.13\linewidth}
p{0.1\linewidth}}
\hline
\textbf{Tasks} & \textbf{T1} \cite{jin2021seqcausal} & \textbf{T2} \cite{jin2021seqcausal} & \textbf{T3} \cite{jin2021seqcausal} & \textbf{T4} \cite{wu2022rasipam} & \textbf{T5} \cite{wu2022rasipam} & \textbf{T6} \cite{linden2023flex} & \textbf{T7} \cite{linden2023flex} \\
\hline
\textbf{Example Excerpt} & \textit{The doctors queried a group of 127 middle-aged patients aging from 50 to 60 who were diagnosed with pneumonia.} & \textit{After several iterations of confirming causalities and model updates,} $\dots$ & \textit{The doctors saved the final causality to the analysis history view.} & \textit{E2 re-ranked the tactics in Tactic View based on the tactical importance} $\dots$ & \textit{Experts applied this merging adjustment and obtained a more accurate estimate of the win rate for this serving tactic.} & \textit{Selected 22 attributes of interest for dimensionality reduction with clustering.} & \textit{Changing the color attribute to sepsis}, $\dots$ \\
\hline
\multirow{2}{*}{\shortstack[l]{\textbf{Plaisant}\\ \textbf{et al.}\\ \cite{plaisant2016diversity}}} & Identify a set of records of interest & Review data quality and inform choices to be made in order to model the data & \textcolor{Red3}{n/a} & \textcolor{magenta}{Identify a set of records of interest} & Review data quality and inform choices to be made in order to model the data & Review data quality and inform choices to be made in order to model the data  & \textcolor{Red3}{n/a} \\
\cline{6-7}
&  &  &  & & Identify a set of records of interest & Identify a set of records of interest &  \\
\hline
\textbf{Du et al. \cite{du2016volumeandvariety}} & Goal-Driven Record Extracting & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} \\
\hline
\multirow{2}{*}{\shortstack[l]{\textbf{Peiris}\\ \textbf{et al.}\\ \cite{peiris2022data}}} & action: Filter\newline target: Event Sequences\newline criteria: Metadata Attributes & action: Derive Metrics\newline target: \textcolor{Red3}{n/a}\newline criteria: \textcolor{Red3}{n/a} & action: \textcolor{magenta}{Annotate}\newline target: \textcolor{Red3}{n/a}\newline criteria: \textcolor{Red3}{n/a} & action: {Sort/Rank}\newline target: \textcolor{magenta}{Event Sequences}\newline criteria: Metrics/Features & action: Add/Modify \textcolor{magenta}\newline target: \textcolor{magenta}{Event Sequences}\newline criteria: Metrics/Features & action: Derive Metrics \newline target: Metadata Attributes \newline criteria: \textcolor{Red3}{n/a} & \textcolor{Red3}{n/a} \\
\cline{7-7}
 & &  & &  &  & action: Group \newline target:\textcolor{Red3}{n/a} \newline criteria: \textcolor{Red3}{n/a} &  \\
\hline
\multirow{2}{*}{\textbf{Ours}} & Intent: Configure Data\newline Strategy: Include-Exclude\newline Technique: Execute Dynamic Queries\newline action: Query\newline input: Event Sequences\newline output: Filtered Event Sequences\newline criteria: Age & Intent: Configure Data\newline Strategy: Refine\newline Technique: Adjust Parameters\newline action: Adjust\newline input: Current causal model\newline output: Updated causal model\newline criteria: Domain knowledge & Intent: Create Provenance\newline Strategy: Document\newline Technique: Save/Record Analysis\newline action: Save/Record\newline input: Analysis State\newline output: Saved/Recorded Analysis\newline criteria: User-specified snapshot & Intent: Configure Visualization\newline Strategy: Rearrange\newline Technique: Reorder/Sort Components\newline action: Reorder/Sort\newline input: Tactics\newline output: Reordered Tactics\newline criteria: Tactical importance metric & Intent: Configure Data\newline Strategy: Refine\newline Technique: Modify Summary\newline action: Modify\newline input: Tactics\newline output: Modified Tactics\newline criteria: Domain knowledge & Intent: Augment Data\newline Strategy: Derive\newline Technique: Obtain Embeddings/Projections\newline action: Obtain\newline input: Attributes\newline output: Projections\newline criteria: t-SNE  & Intent: Configure Visualization\newline Strategy: Visualize\newline Technique: Produce Visualization\\
\cline{7-7}
&  &  &  &  & & Intent: Augment Data\newline Strategy: Organize\newline Technique: \textcolor{magenta}{Group Sequences}\newline action: Group\newline input: \textcolor{Red3}{n/a}\newline output: \textcolor{Red3}{n/a}\newline criteria: clustering & \\
\hline
\end{tabular}}
\end{table*}

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

